Approaching the Quantum Singleton Bound with Approximate Error Correction

It is well known that no quantum error correcting code of rate $R$ can correct adversarial errors on more than a $(1-R)/4$ fraction of symbols. But what if we only require our codes to *approximately* recover the message? We construct efficiently-decodable approximate quantum codes against adversarial error rates approaching the quantum Singleton bound of $(1-R)/2$, for any constant rate $R$. Moreover, the size of the alphabet is a constant independent of the message length and the recovery error is exponentially small in the message length. Central to our construction is a notion of quantum list decoding and an implementation involving folded quantum Reed-Solomon codes.

==> 8-lower-bounds.tex <==
\section{A Robust Quantum Singleton Bound}
\label{sec:lowerbounds}

% \subsection{Non-Private AQECCs}
In this section, we show that the following robust version of the quantum Singleton bound holds for approximate quantum error correction. Such a bound is needed to show that our AQECC construction is optimal, as the ordinary quantum Singleton bound is stated only for exact error correction. Below, we let $H_2$ denote the binary entropy function.

\begin{theorem}
\label{thm:robqsing}
If a $(\delta,\epsilon)$-AQECC of local dimension $q$ encodes $k$ qudits into $n$ qudits, then letting $d=\lfloor\delta n\rfloor+1$, we have
\begin{equation*}
    k \leq n-2(d-1) + 12\sqrt{\epsilon}\cdot n + \frac{H_2(\min\{4\sqrt{\epsilon},1/2\})}{\log_2q}.
    % k \leq n(1-2\delta+12\sqrt{\epsilon})+3.
    % k \leq n - 2(\delta n-1) + 12\sqrt{\epsilon}\cdot n + \frac{1}{\log_2q}.
\end{equation*}
\end{theorem}

When $\epsilon=2^{-\Omega(n)}$ as in our AQECC constructions, \Cref{thm:robqsing} shows that the ordinary quantum Singleton bound $k\leq n-2(d-1)$ holds up to an error of $2^{-\Omega(n)}$. Thus our constructions approach the optimal rate-distance tradeoff as the alphabet size $q$ grows sufficiently large. \Cref{thm:robqsing} also shows that even for small constant $\epsilon$, the quantum Singleton bound holds up to a small error, so we could not hope to improve the rate-distance tradeoff of our AQECCs by allowing a worse recovery error.

The proof of \Cref{thm:robqsing} generally follows the entropy-based proof of the ordinary bound, though more care is needed in dealing with approximate correction and with the classical side channel. A similar argument was outlined in \cite[Section VI]{grassl2022entropic}, but we have not seen a full proof written out in the literature, so we include it here.

We will need the following well-known result. Below we use the notation $\mathcal{B}(\mathcal{H})$ to denote the space of operators on a finite-dimensional Hilbert space $\mathcal{H}$.

\begin{theorem}[Information-disturbance \cite{Kretschmann2008TheIT}]
\label{thm:infdist}
For a quantum channel $\mathcal{X}:\mathcal{B}(A)\rightarrow \mathcal{B}(B)$, let $V:A\rightarrow B\otimes F$ be a Stinespring dilation, and let $\mathcal{X}^c:\mathcal{B}(A)\rightarrow \mathcal{B}(F)$ be the complementary channel. Then there exists some $\sigma\in\mathcal{B}(F)$ such that if $\mathcal{S}:\mathcal{B}(A)\rightarrow\mathcal{B}(F)$ denotes the completely depolarizing channel mapping all inputs to $\sigma$, then 
\begin{equation*}
    \frac14\inf_{\mathcal{D}}\|\mathcal{D}\circ\mathcal{X}-I\|_\diamond^2 \leq \|\mathcal{X}^c-\mathcal{S}\|_\diamond \leq 2\inf_{\mathcal{D}}\|\mathcal{D}\circ\mathcal{X}-I\|_\diamond^{1/2},
\end{equation*}
where the infimum is over all possible decoding channels $\mathcal{D}:\mathcal{B}(B)\rightarrow\mathcal{B}(A)$.
\end{theorem}

\begin{proof}[Proof of \Cref{thm:robqsing}]
  Consider a $(\delta,\epsilon)$-AQECC of local dimension $q$ that maps a message register $A=(\mathbb{C}^q)^{\otimes k}$ to a code register $Q=(\mathbb{C}^q)^{\otimes n}$. Let $\Enc:A\rightarrow Q\otimes F$ be a Stinespring dilation of the encoding channel with environment register $F=(\mathbb{C}^q)^f$. Then $\Enc$ is an isometry, that is $\Enc^\dagger\Enc=I$, and we may assume that $f\leq\log_q(\dim(A)\dim(Q))=k+n$. For a subset $Q'$ of $>(1-\delta)n$ qudits in $Q$, let $\Dec_{Q'}:\mathcal{B}(Q')\rightarrow\mathcal{B}(Q)$ be the channel that fills qudits outside of $Q'$ with a maximally mixed state, and then applies the decoding channel given by the definition of an AQECC.
  
Recall that $d=\lfloor\delta n\rfloor+1$, and let $Q_1$ be the first $d-1$ qudits in $Q$, let $Q_2$ be the next $d-1$ qudits in $Q$, and let $Q_3$ be the remaining $n-2(d-1)$ qudits in $Q$. By definition we have
\begin{equation*}
    \|\Dec_{Q_2Q_3}\circ\Res_{Q_2Q_3}\circ\Enc-I\|_\diamond \leq \epsilon,
\end{equation*}
where $\Res$ denotes restriction to the indicated registers. Then \Cref{thm:infdist} implies that there exists a density matrix $\sigma\in\mathcal{B}(Q_1F)$ such that if $\mathcal{S}:\mathcal{B}(A)\rightarrow\mathcal{B}(Q_1F)$ denotes the channel mapping all its inputs to $\sigma$, then
\begin{equation}
\label{eq:almostconstant}
    \|\Res_{Q_1F}\circ\Enc-\mathcal{S}\|_\diamond = \|(\Res_{Q_2Q_3}\circ\Enc)^c-\mathcal{S}\|_\diamond \leq 2\sqrt{\epsilon}
\end{equation}

Let $\ket{\phi}=\sum_x\ket{x}\ket{x}\in A\otimes A$ be the maximally entangled state, and let $\ket{\psi}=(I\otimes\Enc)\ket{\phi}\in A\otimes Q\otimes F$ be the encoding, where $Q=Q_1\otimes Q_2\otimes Q_3$. Then \Cref{eq:almostconstant} implies the following inequalities:
\begin{align*}
    \|\psi^{AQ_1F}-\psi^A\otimes\sigma^{Q_1F}\|_1 &\leq 2\sqrt{\epsilon} \\
    \|\psi^{Q_1F}-\sigma^{Q_1F}\|_1 &\leq 2\sqrt{\epsilon}.
\end{align*}
Applying the triangle inequality with the above inequalities gives that
\begin{equation*}
    \|\psi^{AQ_1F}-\psi^A\otimes\psi^{Q_1F}\|_1 \leq 4\sqrt{\epsilon}.
\end{equation*}
For a density matrix $\rho$, let $H(\rho)$ denote the von-Neumann entropy of $\rho$ with logarithms taken base $q$. It follows by the Fannes-Audenaert inequality \cite{audenaert2006sharp} that
% Note: the Fannes-Audenaert inequality is actually a little tighter, as it lets us replace the $1/\log_2q$ below with something that also decays with $\epsilon$
\begin{align*}
    |H(AQ_1F)_{\psi^A\otimes\psi^{Q_1F}}-H(AQ_1F)_\psi| 
    &\leq 4\sqrt{\epsilon} \cdot \log_q\dim(AQ_1F)+\frac{H_2(\min\{4\sqrt{\epsilon},1/2\})}{\log_2q}.
\end{align*}
Letting $\epsilon'=H_2(\min\{4\sqrt{\epsilon},1/2\})/\log_2q$, the above inequality becomes
\begin{equation*}
    |H(AQ_1F)_{\psi^A\otimes\psi^{Q_1F}}-H(AQ_1F)_\psi| \leq 16\sqrt{\epsilon}\cdot n + \epsilon'.
\end{equation*}
Thus
\begin{equation*}
    H(A)_\psi+H(Q_1F)_\psi = H(AQ_1F)_{\psi^A\otimes\psi^{Q_1F}} \leq H(AQ_1F)_\psi + 16\sqrt{\epsilon}\cdot n+\epsilon'.
\end{equation*}
Because $H(AQ_1F)_\psi=H(Q_2Q_3)_\psi\leq H(Q_2)_\psi+H(Q_3)_\psi$, it follows that
\begin{equation*}
    H(A)_\psi+H(Q_1F)_\psi \leq H(Q_2)_\psi+H(Q_3)_\psi + 16\sqrt{\epsilon}\cdot n+\epsilon'.
\end{equation*}

Now observe that we may choose to provide the decoding channel with the register $F$, so that similarly to \Cref{eq:almostconstant}, we have
\begin{equation*}
    \|\Res_{Q_1}\circ\Enc-\mathcal{S}\|_\diamond = \|(\Res_{Q_2Q_3F}\circ\Enc)^c-\mathcal{S}\|_\diamond \leq 2\sqrt{\epsilon}.
\end{equation*}
Following through the same reasoning as above, we obtain that
\begin{equation*}
    H(A)_\psi+H(Q_1)_\psi \leq H(Q_2F)_\psi+H(Q_3)_\psi + 8\sqrt{\epsilon}\cdot n+\epsilon',
\end{equation*}
where we have a factor of $8\sqrt{\epsilon}$ instead of $16\sqrt{\epsilon}$ as before because $\log_q\dim(AQ_1)\leq 2n$. By symmetry of $Q_1$ and $Q_2$, we similarly have that
\begin{align*}
    H(A)_\psi+H(Q_2F)_\psi &\leq H(Q_1)_\psi+H(Q_3)_\psi + 16\sqrt{\epsilon}\cdot n+\epsilon' \\
    H(A)_\psi+H(Q_2)_\psi &\leq H(Q_1F)_\psi+H(Q_3)_\psi + 8\sqrt{\epsilon}\cdot n+\epsilon'.
\end{align*}
Averaging the four inequalities we showed above gives that
\begin{equation*}
    H(A)_\psi \leq H(Q_3) + 12\sqrt{\epsilon}\cdot n + \epsilon'.
\end{equation*}
By construction $H(A)_\psi=k$ and $H(Q_3)\leq n-2(d-1)$, so the desired result follows.
\end{proof}

% \subsection{Private AQECCs}

% \louis{Need to figure out what the optimal result is; problem is that encoder may perform arbitrary POVM on environment register $F$, which then could require a Hilbert space of arbitrarily large dimension, which in turn incurs a big loss from the application of Fannes inequality.}

% \begin{figure}
%   \centering
%   \begin{subfigure}{.8\textwidth}
%     \begin{quantikz}
%       \lstick[wires=2]{$\ket{\phi}=\sum_x\ket{x}\ket{x}$} & \qw{A} & \qw & \qw & \qw & \qw & \qw & \qw & \qw \rstick[wires=2]{$\approx\ket{\phi}$} \\
%       & \qw{A'} & \gate[wires=4,nwires={2}]{\Enc} & \qw{Q_1} & \qw & \qw & \qw & \gate[wires=3,cwires={3}]{\Dec} & \qw \\
%       & & & \qw{Q_2} & \gate[swap,style={draw=none}]{} & \qw & \qw & \qw \\
%       \lstick{$\ket{0^{n-k}}$} & \qw & & \qw{Q_3} & \qw & \gate[swap,style={draw=none}]{} & \meter{} & & \qw \\
%       \lstick{$\ket{0^f}$} & \qw & & \qw{F} & \qw & & \qw & \qw & \qw \\
%     \end{quantikz}
%     \caption{\label{fig:decmeas} Decoding a private AQECC when register $Q_2$ is erased from the code state. Registers $A$ and $A'$ are $k$-qudit message registers initialized with a maximally entangled state $\ket{\phi}$ across them. The encoding circuit takes as input the message in $A'$, as well as $n-k+f$ ancillas, and outputs the code state in the $n$-qudit register $Q=Q_1Q_2Q_3$, which may be entangled with the $f$-qudit environment register $F$. Here $Q$ is partitioned into $(d-1)$-qudit registers $Q_1,Q_2$ and $(n-2(d-1))$-qudit register $Q_3$. We assume without loss of generality that the private classical channel is used to send the decoder the entire measurement outcome of the environment register $F$.}
%   \end{subfigure}
%   \begin{subfigure}{.8\textwidth}
%     \begin{quantikz}
%       \lstick[wires=2]{$\ket{\phi}=\sum_x\ket{x}\ket{x}$} & \qw{A} & \qw & \qw & \qw & \qw & \qw & \qw \rstick[wires=2]{$\approx\ket{\phi}$} \\
%       & \qw{A'} & \gate[wires=4,nwires={2}]{\Enc} & \qw{Q_1} & \qw & \qw & \gate[wires=3]{\Dec} & \qw \\
%       & & & \qw{Q_2} & \gate[swap,style={draw=none}]{} & \qw & \qw \\
%       \lstick{$\ket{0^{n-k}}$} & \qw & & \qw{Q_3} & \qw & \gate[swap,style={draw=none}]{} & \qw & \qw \\
%       \lstick{$\ket{0^f}$} & \qw & & \qw{F} & \ctrl{1} & & \qw & \qw \\
%       \lstick{$\ket{0^f}$} & \qw & \qw & \qw & \targ{} & \qw{M} & \qw & \qw
%     \end{quantikz}
%     \caption{\label{fig:decnomeas} An equivalent decoding circuit that delays the measurement by entangling the environment register $F$ with another register $M$.}
%   \end{subfigure}
% \end{figure}


==> 9-erasure-qec.tex <==
\section{Worst to Random Case Pauli Error QLD }

We use a theorem by Rudra

\begin{theorem}\label{theorem:rudra}
    Let $\epsilon, \delta$ be reals and let $q$ and $n >\Omega(1/\epsilon)$  be positive integers. Let $C$ be a $[n, k, \delta\cdot n]_q$ code. Let $0<\rho<\delta-\epsilon$ be a real.  Let $S\subset [n]$ with $|S| = (1 - \rho)n$. Then if $q = 2^{\Omega(1/\epsilon)}$, for every codeword $c$ and all but a $q^{-\Omega(\epsilon n)}$ fraction of error patterns $e \in \Sigma$ with $wt(e) = \rho n$ and $wt_S(e) = 0$, the only codeword within the Hamming ball of radius $\rho n$ around the received word $c + e$ is $c$.
\end{theorem}

\begin{remark}
    If $|S| = (1-\delta+\epsilon)\cdot n$ and $q = 2^{\Omega(1/\epsilon)}$, then for all but a $q^{-\Omega(\epsilon n)}$ fraction of error patterns $e \in \Sigma$ with $wt(e) < (\delta-\epsilon) n$ and $wt_S(e) = 0$, the only codeword within the Hamming ball of radius $\rho n$ around the received word $c + e$ is $c$.
\end{remark}

We note that by \Cref{theorem:rudra}, for all but an exponentially small fraction of errors $e$ on region of size $\leq (\delta-\epsilon)n$, $|B(c+e, (\delta-\epsilon))\cap C|=1$. Thus we can define a classical algorithm $\mathbb{A}_C(c+e)$ which (takes exponential time and) for most $e$, finds the unique correction $\hat{e} = -e$ to any codeword of distance $(\delta-\epsilon)n$ away from $c+e$. We allow $\mathcal{A}_C$ to output the first valid correction $\hat{e}$ ($c+e+\hat{e}\in C$) if otherwise. Following section LD, let $V_C$ be the unitary which computes and adds $\mathcal{A}_C$:

\begin{equation}
    V_C \big(|c+e\rangle |0^{anc}\rangle \big) = |c+e\rangle |\mathcal{A}_C(c+e)\rangle 
\end{equation}

We show how to use the $V_C$ of classical linear codes in a CSS code to decode quantum codes from Random Paulis.

\begin{lemma} \label{lemma:randompaulis}
Consider a $[n, k, \delta\cdot n]_q$ QECC $Q$, defined via the CSS code of two classical codes $C_1, (C_2)^\perp$ of distance $d$. Fix $\rho<\delta-\epsilon$ and a subset $S\subset [n]$ of size $|S| = (1-\rho)n$ of qudits, and consider the subset $\mathcal{P}_S$ of all $n$-qudit Paulis $\mathcal{P}_q^{\otimes n}$ of weight $0$ on $S$ and $\rho\cdot n$ on $[n]\setminus S$. Then there exists a unitary $\mathcal{D}$ which for all but a $1-q^{-\Omega(\epsilon n)}$ fraction of Pauli errors $E$ in $P_S$, 

\begin{equation}
    \mathcal{D} (E\otimes \mathbb{I}_{S, anc}) |\psi\rangle |0^{anc}\rangle  = |\psi\rangle \otimes |aux\rangle 
\end{equation}

$\forall \psi \in Q$.
\end{lemma}

\begin{proof}
    Consider a Pauli operator $X^{a}_qZ^b_q\in  \mathcal{P}_S$. Let $\mathcal{D}$ perform the quantum list decoding algorithm of claim \Cref{claim:CSS}, using the unitaries $V_{C_1}, V_{(C_2)^\perp}$ guaranteed by theorem \Cref{theorem:rudra} and the  discussion above.
    
    %we define $\mathcal{D}$ to attempt to decode the Pauli error using $V_{C_1}$, changing basis, applying $V_{(C_2)^\perp}$, and changing basis again. Via the translational invariance of the linear code (\Cref{fact-invariant}) we know the corrections $\hat{e}_1, \hat{e}_2$ output by the decoding unitaries $V$ only depend on $a, b$, so we restrict our attention to a basis vector $|\bar{x}\rangle$ of the codespace. 
    
    After which, the algorithm concludes by applying a Pauli `correction' controlled on the description in the list (of a single element), i.e.

    \begin{equation}
        |x\rangle |\hat{e}_1\rangle |\hat{e}_2\rangle\rightarrow Z_q^{\hat{e}_2} X_q^{\hat{e}_1}|x\rangle |\hat{e}_1\rangle |\hat{e}_2\rangle = \omega^{\hat{e}_2\cdot (x+\hat{e_1})} |x+\hat{e}_1\rangle |\hat{e}_1\rangle |\hat{e}_2\rangle
    \end{equation}

   \noindent In this setting 
    \begin{equation}
        \mathcal{D} (X^aZ^b\otimes \mathbb{I}_{S, anc}) |\psi\rangle |0\rangle =   |\psi\rangle |\hat{e}_1\rangle |\hat{e}_2\rangle
    \end{equation}

    \noindent if $\hat{e}_1 = -a$ and $\hat{e}_2=-b$. From theorem \Cref{theorem:rudra}, we know that this occurs for all but a $q^{-\Omega(\epsilon n)}$ fraction of all $a$ (resp $b$) of weight $\leq \rho\cdot n$ on $S$. This implies that for all but a $2\cdot q^{-\Omega(\epsilon n)}$ fraction of Pauli operators $E=X^aZ^b\in \mathcal{P}_S$ of weight $\leq (\delta-\epsilon)\cdot n$ on $[n]\setminus S$, $\mathcal{D}$ recovers $\psi$ exactly. 
    
    Finally, consider the set of Pauli $\mathcal{P}_{S, \rho}$ errors of weight \textit{exactly} $\rho\cdot n = |[n]\setminus S|$ on $S^C\subset [n]$. We note that 

    \begin{equation}
        \frac{|\mathcal{P}_{S, \rho}|}{|\mathcal{P}_{S}|} \geq  (1-1/q^2)^{n} \geq e^{-O(n/q^2)} 
    \end{equation}

    \noindent since the only pairs $a',b' \in \mathcal{P}_{S} \setminus \mathcal{P}_{S, \rho}$ are those which exists a location $i$ with $a'_i=b'_i=0$. Note that the ratio above is at least the probability a random $(a', b')\in \mathcal{P}_{S}$ has for all $i$ that either $a'_i, b'_i\neq 0$. Thus, we also have that for all but a  

    \begin{equation}
       \frac{1}{|\mathcal{P}_{S, \rho}|} \cdot \bigg(q^{-\Omega(\epsilon n)} \cdot |\mathcal{P}_{S}|\bigg) \leq  e^{O(n/q^2)} q^{-\Omega(\epsilon n)} = q^{-\Omega(\epsilon n)}
    \end{equation}

fraction of errors in $\mathcal{P}_{S, \rho}$, $\mathcal{D}$ decodes exactly. In the above recall we assume $q>2^{\Omega(1/\epsilon)}$.
    
\end{proof}

Sample random single qudit clifford gates $C_1\cdots C_n$, and apply each gate on the corresponding physical qudit of the QECC. We claim that this defines an AQECC, secure against oblivious adversaries - those who don't know the $C_i$. Later, we remove this assumption using a classical side register. 

\begin{theorem}
    Assume $q>2^{\Omega(1/\epsilon)}$. The quantum code defined by the concatenation of a $[n, k, d]_q$-QECC with random single qudit clifford gates is AQECC up to radius $d(1-\epsilon)$ with fidelity $1-q^{-\Omega(\epsilon \cdot n)}$.
\end{theorem}


We prove this claim in several steps. First, we define a recovery channel which corrects fixed Pauli errors. Then, we argue that correcting Pauli Errors approximately suffices to correct an arbitrary adversarial quantum error channel. Define the channel $\mathcal{R}$ to first decrypt the random cliffords, then apply $\mathcal{D}$ as guaranteed in lemma \Cref{lemma:randompaulis}, and finally trace out the output on the list register and ancillas. I.e., 

\begin{equation}
    \mathcal{R}(\rho) = \text{Tr}_{[n]^C}\big[\mathcal{D}\circ (\bigotimes_i  C_i^\dagger \otimes \mathbb{I}_{[n]^C})\circ \rho]
\end{equation}

Let $\rho_{a, b} = \mathbb{E}_{C_1\cdots C_n} \mathcal{R}(X^aZ^b \circ \otimes_{i\in [n]}C_i \circ \psi) $ define the output density matrix of the recovery channel, over random choice of cliffords $C_1\cdots C_n$, for a fixed Pauli error $X^aZ^b$ of weight $\rho n < (\delta-\epsilon)\cdot n$. The fidelity of $\rho_{a, b}$ with $\psi$ approaches $1$ exponentially quickly:

\begin{claim}
The fidelity $F (\rho_{a, b}, \psi) = \langle \psi|\rho_{a, b}|\psi\rangle \geq 1-q^{-\Omega(\epsilon \cdot n)}$
\end{claim}

\begin{proof}
Let $X^{\Tilde{a}}Z^{\Tilde{b}} =  (\bigotimes_i  C_i^\dagger) X^aZ^b (\bigotimes_i  C_i^\dagger)$, where $X^{\Tilde{a}}, Z^{\Tilde{b}}$ are $n$ qudit Paulis. Recall that conjugation by Clifford gates is an injective map from $n$ qudit Paulis to $n$ qudit Paulis, by definition. Consider first the action of the decoding channel, on the corrupted state $|\psi'\rangle = X_q^aZ_q^b|\psi\rangle$. Thus except for an exponentially small fraction of $a, b$, before tracing out the list register, we receive the pure state

\begin{equation}
    \mathcal{D}(\bigotimes_i  C_i^\dagger \otimes \mathbb{I}_{[n]^C})|\psi'\rangle|0^{anc}\rangle = \mathcal{D} (X^{\Tilde{a}}Z^{\Tilde{b}} \otimes \mathbb{I}_{[n]^C}) |\psi\rangle |0^{anc}\rangle = |\psi\rangle \otimes |-\Tilde{a}\rangle |-\Tilde{b}\rangle
\end{equation}

Let $Bad_S\subset \mathcal{P}_{S, \rho}$ denote the bad subset of Pauli Errors guaranteed by lemma \Cref{lemma:randompaulis}, on which we have no guarantees on the decoding algorithm $\mathcal{D}$. Recall $S = Supp(X^aZ^b), wt(X^aZ^b) = \rho\cdot n$. The reduced density matrix $\rho_{a, b}$ output by $\mathcal{R}$ can be expressed as
\begin{gather}
    \rho_{a, b} = \mathbb{E}_{C_1\cdots C_2}\bigg( \mathcal{R}(X^a_q Z^b_q\circ \otimes_{i\in [n]}C_i \circ \psi) \bigg)  =\\ = \mathbb{E}_{C_1\cdots C_2}\bigg[ \mathbb{I}_{(\Tilde{a},\Tilde{b})\in  Bad_S} \cdot \rho_{Failed} + \mathbb{I}_{(\Tilde{a},\Tilde{b})\notin  Bad_S} \cdot \psi\bigg] = \\ = \psi \cdot \mathbb{P}_{C_1\cdots C_n}[(\Tilde{a}, \Tilde{b}) \notin Bad_S] + \rho_{Failed}\cdot \mathbb{P}_{C_1\cdots C_n}[(\Tilde{a}, \Tilde{b}) \in Bad_S]
\end{gather}

We note that if $E = X^a_q Z^b_q\in \mathcal{P}_{S, \rho}$, then $X^{\Tilde{a}}Z^{\Tilde{b}}$ is a uniformly random element of $\mathcal{P}_{S, \rho}$. That is, a Random Pauli of weight $\rho\cdot n < (\delta-\epsilon)\cdot n$, wt$_{S}(E) = 0$. Thus

\begin{equation}
    \mathbb{P}_{C_1\cdots C_n}[(\Tilde{a}, \Tilde{b}) \in Bad_S] = \frac{|Bad_S|}{|\mathcal{P}_{S, \rho}|}\leq q^{-\Omega(\epsilon n)}.
\end{equation}

\end{proof}


\begin{claim}
    Let $Adv_S(\psi) = \sum_i K_i^\dagger \psi K_i$ be an adversarial quantum channel defined by Kraus operators $\{K_i\}$ supported on a subset $S\subset [n]$ of size $|S|\leq n(\delta-\epsilon)$. Then, for any $\psi$ in the QECC $Q$, the density matrix $\rho_{Adv} =\mathbb{E}_{C_1\cdots C_n}\mathcal{R}\circ Adv_S\circ \otimes_{i\in [n]}C_i \circ \psi$ output by the recovery channel $\mathcal{R}$ satisfies

    \begin{equation}
        F(\rho_{Adv}, \psi) \geq 1- q^{-\Omega(\epsilon\cdot n)}
    \end{equation}
\end{claim}

\begin{proof}
    We note $F(\rho_{Adv}, \psi)$ decomposes into a sum over Krauss operators, so for now let us restrict our attention to a fixed $K_i = K = \sum_{\sigma\in \mathcal{P}_{S}} c_\sigma \sigma$. Furthermore, fix the choice of random cliffords $\{C_i\}$, which later we average over. The decoding unitary $\mathcal{D}$ acts on $K$ by list decoding its Pauli basis decomposition in superposition:
    \begin{gather}
        \mathcal{D}\bigg(\otimes_{i\in [n]}C_i^\dagger\bigg) K \bigg(\otimes_{i\in [n]}C_i \bigg) \psi = \sum_{(a, b)\in \mathcal{P}_{S}} c_{(a,b)} Z^{e_2^b}_qX^{e_1^a}_q X^{\Tilde{a}}_qZ^{\Tilde{b}}_q \ket{\psi} \ket{e^{\Tilde{a}}_1} \ket{e^{\Tilde{b}}_2} = \\ = |\psi\rangle \sum_{(a, b) \in \mathbb{P}_S: (\Tilde{a}, \Tilde{b}) \notin Bad_S} c_{(a,b)} \ket{e^{\Tilde{a}}_1} \ket{e^{\Tilde{b}}_2}  + \sum_{(a, b) \in \mathbb{P}_S: (\Tilde{a}, \Tilde{b}) \in Bad_S} c_{(a,b)} |junk_{a,b}\rangle \ket{e^{\Tilde{a}}_1} \ket{e^{\Tilde{b}}_2} 
    \end{gather}

    where once again the superscripts $\Tilde{a}, \Tilde{b}$ denote the clifford conjugated Paulis, and recall $e^{\Tilde{a}}_1$ is the correction defined by $\Tilde{a}$. In this sense, we observe that $\mathcal{D}$ has written out a (possibly incorrect) `correction' for the Pauli errors in $K$ in superposition. 
    
    Now, let us consider the next step in $\mathcal{R}$, tracing out the list register. The key observation is that not many pairs of Pauli errors contain the exact same correction in their list. In fact, if $(\Tilde{a}, \Tilde{b}) \notin Bad_S$, then its correction doesn't overlap with any other error $(\Tilde{a}', \Tilde{b}') \notin Bad_S$. 

    \begin{equation}
       \mathcal{R}(K\circ\big(\otimes_{i\in [n]}C_i \big) \circ \psi) = \sum_{ (a,b), (a',b')\in \mathcal{P}_{S}} c_{a, b}c^*_{a',b'} \mathbb{I}[ e_1^{\Tilde{a}}= e_1^{\Tilde{a}'} \text{ and } e_2^{\Tilde{b}}= e_2^{\Tilde{b}'}] \cdot \ket{\psi_{a, b}}\bra{\psi_{a', b'}} =
    \end{equation}

    where $\ket{\psi_{a, b}} = \ket{\psi}$ if $(\Tilde{a}, \Tilde{b}) \notin Bad_S$ and $|junk_{a,b}>$ otherwise. Let $Good_{S}\subset \mathcal{P}_S$ denote the set of Paulis whose corrections $e_1^a, e_2^b$ are unique: i.e. $\nexists (a',b')\in \mathcal{P}_S$ s.t. $(a', b')\neq (a, b)$ and $(e_1^a, e_2^b)=(e_1^{a'},e_2^{b'})$. We note that $|Good_{S}| \geq |\mathcal{P}_S|- 2|Bad_S| \geq (1-q^{-\Omega(\epsilon\cdot n)})$, as the corrections of the errors in $Bad_S$ can overlap with the corrections of at most $Bad_S$ elements of $|\mathcal{P}_S\setminus Bad_S|$. Thus,

    \begin{equation}
        = |\psi\rangle \langle \psi| \cdot \bigg(\sum_{\substack{(a,b)\in \mathcal{P} \\ 
                \Tilde{a},  \Tilde{b}\in Good_S}} |c_{(a, b)}|^2 \bigg) + \rho_{Junk}
    \end{equation}

    Now, in expectation over the choice of random Cliffords, 

    \begin{equation}
        \rho_{Adv}^K =\mathbb{E}_{C_1\cdots C_n} \mathcal{R}(K\circ\big(\otimes_{i\in [n]}C_i \big) \circ \psi) = \psi \cdot \bigg( \sum_{(a,b)\in \mathcal{P}_S\}} |c_{a,b}|^2 \cdot \mathbb{P}_{C_1\cdots C_n}[\Tilde{a},\Tilde{b}\in Good_S]\bigg) + \rho_{Junk'} 
    \end{equation}

    where we note that $\mathbb{P}_{C_1\cdots C_n}[\Tilde{a},\Tilde{b}\in Good_S] $ 

    \textit{not finished}

    
\end{proof}


